HyperExpan: Taxonomy Expansion with Hyperbolic Representation Learning

Taxonomies are valuable resources for many applications, but the limited coverage due to the expensive manual curation process hinders their general applicability. Prior works attempt to automatically expand existing taxonomies to improve their coverage by learning concept embeddings in Euclidean space, while taxonomies, inherently hierarchical, more naturally align with the geometric properties of a hyperbolic space. In this paper, we present HyperExpan, a taxonomy expansion algorithm that seeks to preserve the structure of a taxonomy in a more expressive hyperbolic embedding space and learn to represent concepts and their relations with a Hyperbolic Graph Neural Network (HGNN). Specifically, HyperExpan leverages position embeddings to exploit the structure of the existing taxonomies, and characterizes the concept profile information to support the inference on unseen concepts during training. Experiments show that our proposed HyperExpan outperforms baseline models with representation learning in a Euclidean feature space and achieves state-of-the-art performance on the taxonomy expansion benchmarks.

==> content/3_not_used_sens.tex <==
% \subsection{GNN}
% \label{subsec:match1}

% \begin{figure}[ht!]
% \centering
%     \includegraphics[width=0.95\columnwidth]{figs/org_gnn.png}
%     \caption{
%         \footnotesize
%         \textbf{Applying GNN for taxonomy expansion:} The original TaxoExpan framework utilizes a local \textbf{Ego-Network} for applying the graph neural network (GNN) model to extract node-level features, and then the query would be compared to these aggregated features for the final slot-to-put predictions. Image courtesy: the TaxoExpan paper~\cite{Shen2020TaxoExpanST}.
%     }
%     \label{fig:org_gnn}
% \end{figure}

% As illustrated in Figure~\ref{fig:org_gnn}, the input existing taxonomy (the leftmost tree) can be viewed as a graph, where the vertices (nodes) are the concepts, and the edges represent whether they are hierarchically linked. The edges are directed edge, where the direction indicates a parent-child relationship within the taxonomy, \textit{ie.} suppose $u, v$ are the concept nodes, and that $u \rightarrow v$, then $u$ is the \textit{parent concept} of $v$, \textit{eg.} \textit{Hardware} is the parent concept of \textit{Integrated Circuit} as the former concept encompasses the latter one. Following this definition, an \textbf{Ego Network} with a central \textit{anchor} concept can be extracted, where the closest nearby edges will link to the related concepts of this anchor node. A graph neural network (GNN) can then be applied to encode this ego-network to produce a feature vector (purple vector) to be compared against a query vector embedding a to-be-expanded concept. A followed-up matching module can be then be trained to produce the final slot-putting results for this query concept to be properly expanded.
% The encoder for this ego-network, can be any type of network in the GNN family, including conventional GCN, and attention-based GAT. We will describe a new type of GCN which operates in the hyperbolic space, in the next section.

% \subsection{Hyperbolic GCN}
% \label{subsec:match2}

% \begin{figure}[ht!]
% \centering
%     \includegraphics[width=0.7\columnwidth]{figs/hyper.png}
%     \caption{
%         \footnotesize
%         \textbf{HGCN aggregation method:} we first map the messages/embeddings to the Euclidean tangent space, and then perform the GNN aggregation in such tangent space, and then project them back to the hyperbolic space.
%     }
%     \label{fig:hgcn_agg}
% \end{figure}

% \noindent As derived in~\cite{Chami2019HyperbolicGC}, one can map a Euclidean feature $x^{0, E} \in \mathbb{R}^{d}$ ($E$ denotes the \textit{Euclidean} here.) via an exponential transformation to the hyperbolic space (plane), $\mathbb{H}^{d, K}$, where $d$ is the dimension of the hyperbolic space and that $-1/K$ is the negative curvature of the space, as follows:

% \begin{equation}
%     \mathbf{x}^{0, H}=\exp _{\mathbf{o}}^{K}\left(\left(0, \mathbf{x}^{0, E}\right)\right)=\left(\sqrt{K} \cosh \left(\frac{\left\|\mathbf{x}^{0, E}\right\|_{2}}{\sqrt{K}}\right), \sqrt{K} \sinh \left(\frac{\left\|\mathbf{x}^{0, E}\right\|_{2}}{\sqrt{K}}\right) \frac{\mathbf{x}^{0, E}}{\left\|\mathbf{x}^{0, E}\right\|_{2}}\right)
% \end{equation}

% Figure~\ref{fig:hgcn_agg} illustrates the transformation in some exemplar spaces.

% The above mathematical transformation is used in the HGCN module to map the embedding space of a particular layer to the next layer and cope with the neighboring structure of a given graph. And hence, we need to also mathematically define the usual matrix multiplication and bias addition mechanism in such a hyperbolic space, also via the exponential transformation tricks.
% We can first use the \textit{logarithmic} transformation to project the hyperbolic point $x^H$ to the tangent plane $\mathcal{T}_{\mathbf{o}} \mathbb{H}^{d, K}$, and then we can properly define the aforementioned atomic operations in every kind of neural networks, in the tangent space.
% And finally, a simple exponential transformation is required to map the multiplication results back to the hyperbolic space, as illustrated below:

% \begin{equation}
%     W \otimes^{K} \mathbf{x}^{H}:=\exp _{\mathbf{o}}^{K}\left(W \log _{\mathbf{o}}^{K}\left(\mathbf{x}^{H}\right)\right)
% \end{equation}

% And likewise, we can define the operation for bias addition, with the help of parallel transport (see Figure~\ref{fig:hgcn_agg}), denoted by the $\rightarrow$ as below: 

% \begin{equation}
%     \mathbf{x}^{H} \oplus^{K} \mathbf{b}:=\exp _{\mathbf{x}^{\mathbf{H}}}^{K}\left(P_{\mathbf{o} \rightarrow \mathbf{x}^{H}}^{K}(\mathbf{b})\right)
% \end{equation}

% As now we have properly mathematically define the necessary operations, the usual attention-based aggregation mechanism in a graph attention network (GAT)~\cite{velivckovic2017graph} can be reformulated as follows:

% \begin{equation}
% \begin{aligned}
%     w_{i j} &=\operatorname{SoFTMAX}_{j \in \mathcal{N}(i)}\left(\mathbf{M L P}\left(\log _{\mathbf{o}}^{K}\left(\mathbf{x}_{i}^{H}\right) \| \log _{\mathbf{o}}^{K}\left(\mathbf{x}_{j}^{H}\right)\right)\right) \\
%     \mathrm{AGG}^{K}\left(\mathbf{x}^{H}\right)_{i} &=\exp _{\mathbf{x}_{i}^{H}}^{K}\left(\sum_{j \in \mathcal{N}(i)} w_{i j} \log _{\mathbf{x}_{i}^{H}}^{K}\left(\mathbf{x}_{j}^{H}\right)\right)
%     \end{aligned}
% \end{equation}

% On the other hand, a non-linear (in the Euclidean space) activation function can be formulated as:

% \begin{equation}
%     \sigma^{\otimes^{K_{\ell-1}, K_{\ell}}}\left(\mathbf{x}^{H}\right)=\exp _{\mathbf{o}}^{K_{\ell}}\left(\sigma\left(\log _{\mathbf{o}}^{K_{\ell-1}}\left(\mathbf{x}^{H}\right)\right)\right)
% \end{equation}

% Finally, we can derive the formulas for the hyperbolic variant of the GCN.
% HGCN essentially can stack multiple hyperbolic GCN layers, where at each layer HGCN
% first preform the hyperbolic transformation and then conduct the corresponding aggregation to incorporate neighbor’s embeddings in the tangent space of the center node.
% And, hence the hyperbolic message passing in a HGCN layer is derived as:

% \begin{equation}
% \begin{aligned}
%     &\mathbf{h}_{i}^{\ell, H}=\left(W^{\ell} \otimes^{K_{\ell-1}} \mathbf{x}_{i}^{\ell-1, H}\right) \oplus^{K_{\ell-1}} \mathbf{b}^{\ell} \quad \text { (hyperbolic feature transform) }\\
%     &\mathbf{y}_{i}^{\ell, H}=\mathrm{AGG}^{K_{\ell-1}}\left(\mathbf{h}^{\ell, H}\right)_{i} \quad \text { (attention-based neighborhood aggregation) }\\
%     &\mathbf{x}_{i}^{\ell, H}=\sigma^{\otimes^{K_{\ell-1}, K_{\ell}}}\left(\mathbf{y}_{i}^{\ell, H}\right) \quad \text { (non-linear activation with different curvatures) }
%     \end{aligned}
% \end{equation}


% \subsection{Position-aware Hyperbolic GCN}
% \label{subsec:match3}

% Every input example consists of three types of nodes: 
% \begin{itemize}
%     \item The query node, i.e. the new concept to be inserted into the taxonomy.
%     \item The anchor nodes, i.e. the candidate concept to which the new concept could append.
%     \item The sibling nodes, i.e. the neighbors of the anchor node
% \end{itemize}

% To distinguish the three types of nodes, we enhance the representation of each node at every layer by concatenating an additional type embedding:
% \begin{equation}\mathbf{x'}_i^{l, H} = [\mathbf{x}_i^{l, H}; HypEmb^l(t_i)].\end{equation}

% $t_i$ is the type of node $i$: 
% \begin{equation}
% t_i=
% \begin{cases}
% 0, & \text{ $x_i$ is the query node } \\
% 1, & \text{ $x_i$ is the anchor node } \\
% 2, & \text{ $x_i$ is a neighbor of the anchor node } \\
% \end{cases}
% \end{equation}

% $HypEmb^l$ is the type embedding of $l$-th layer, where we first embed the type into Euclidean space and then project it into the hyperbolic space, similar to how we project $\mathbf{x}^E$ into the hyperbolic space.
